DeepVoxNet2: Yet another CNN framework

We know that both the CNN mapping function and the sampling scheme are of paramount importance for CNN-based image analysis. It is clear that both functions operate in the same space, with an image axis $\mathcal{I}$ and a feature axis $\mathcal{F}$. Remarkably, we found that no frameworks existed that unified the two and kept track of the spatial origin of the data automatically. Based on our own practical experience, we found the latter to often result in complex coding and pipelines that are difficult to exchange. This article introduces our framework for 1, 2 or 3D image classification or segmentation: DeepVoxNet2 (DVN2). This article serves as an interactive tutorial, and a pre-compiled version, including the outputs of the code blocks, can be found online in the public DVN2 repository. This tutorial uses data from the multimodal Brain Tumor Image Segmentation Benchmark (BRATS) of 2018 to show an example of a 3D segmentation pipeline.

==> figures/deconvolution.tex <==
\begin{figure}[b]
    \newcommand\myscale{\scaleppt} %0.55
    \setlength\tabcolsep{0pt}
    \centering
    \includegraphics[scale=\scale,scale=\myscale]{\rootpath figures/files/deconvolution.pdf}
    \caption[Perfusion imaging and deconvolution.]{Perfusion imaging acquires a series of images between t\textsubscript{s} and t\textsubscript{e} after the injection of a contrast agent at t\textsubscript{0}. The measured \gls{tcc}s will look different across different patients and measurements, even so for the injection location itself and for the location of the \gls{aif} at the entrance of the brain. Measurements can be normalized, i.e. \gls{tcc}\textsubscript{\gls{irf}}, by deconvolution, as if they were the result of an \gls{aif}\textsubscript{\gls{imp}}. Straightforwardly, the timing of the start t\textsubscript{s}-t\textsubscript{0} and end t\textsubscript{e}-t\textsubscript{0} of the scan is of crucial importance. The time resolution $\Delta$t is important for the deconvolution to be mathematically valid. From the resulting \gls{tcc}\textsubscript{\gls{irf}}s certain perfusion dynamics can be derived directly.}
    \label{fig:deconvolution}
\end{figure}

==> figures/machine_learning.tex <==
\begin{figure}[t]
    \newcommand\myscale{\scaleppt} %0.55
    \setlength\tabcolsep{0pt}
    \centering
    \includegraphics[scale=\scale,scale=\myscale]{\rootpath figures/files/machine_learning.pdf}
    \caption[A schematic representation of data-driven methods in \gls{ais}.]{Data-driven methods for automated tissue status segmentation in \gls{ais} need (i) a dataset of input-output pairs, and (ii) a model that maps an input to an output. The model has trainable parameters that are tuned (iteratively) to minimize the loss between the observed and predicted output. Current methods mostly provide models for different subsets of the original dataset, e.g. one for core and one for penumbra estimation, respectively using a dataset of reperfusers and non-reperfusers.}
    \label{fig:machine_learning}
\end{figure}

==> figures/progression.tex <==
\begin{figure}[t]
    \newcommand\myscale{\scaleppt}
    \setlength\tabcolsep{0pt}
    \centering
    \begin{tabular}{ccc}
        \multicolumn{3}{c}{\includegraphics[scale=\scale,scale=\myscale]{\rootpath figures/files/progression.pdf}}
    \end{tabular}
    \begin{tabular}{ccc}
        \includegraphics[scale=\scale,scale=\myscale,trim={0 0 0 -0.5cm},clip]{\rootpath figures/files/progression_heads_A.pdf}
        &\includegraphics[scale=\scale,scale=\myscale,trim={-1cm 0 -1cm -0.5cm},clip]{\rootpath figures/files/progression_heads_B.pdf}
        &\includegraphics[scale=\scale,scale=\myscale,trim={0 0 0 -0.5cm},clip]{\rootpath figures/files/progression_heads_C.pdf}
    \end{tabular}\\
    \begin{tabular}{ccc}
        \includegraphics[scale=\scale,scale=\myscale,trim={0 1cm 0 0},clip]{\rootpath figures/files/progression_heads_Dpos.pdf}
        &\includegraphics[scale=\scale,scale=\myscale,trim={-1cm 1cm -1cm 0},clip]{\rootpath figures/files/progression_heads_D.pdf}
        &\includegraphics[scale=\scale,scale=\myscale,trim={0 1cm 0 0},clip]{\rootpath figures/files/progression_heads_Dneg.pdf} 
    \end{tabular}
    \caption[Progression of core and penumbra in \gls{ais}.]{At the onset of an \gls{ais} there is no irreversible damage (A). After a certain \gls{tso}, the patient is triaged for a certain treatment, a.o. based on acute imaging and estimates of the tissue state (i) at that moment (B), and (ii) at the moment when the (partial) reperfusion takes place, i.e. after a certain \gls{ttt} (C). The treatment affects the extent of the final infarction (D- > D > D+) and may slow down the progression (decreasing the tissue hypoperfusion will suppress its malicious effect on surrounding tissue). To assess the final infarction, follow-up imaging should be acquired not sooner than when the infarction has fully progressed (D+).}
    \label{fig:progression}
\end{figure}


==> figures/thresholds.tex <==
\begin{figure}[b]
    \newcommand\myscale{\scaleppt}
    \setlength\tabcolsep{0pt}
    \centering
    \includegraphics[scale=\scale,scale=\myscale]{\rootpath figures/files/thresholds.pdf}
    \caption[Important \gls{cbf} thresholds.]{During a pathological state of cerebral perfusion, the \gls{cbf} decreases progressively. It turns out that \gls{cbf} levels correlate with irreversible and reversible tissue damage. Nevertheless, absolute thresholds vary across different subjects, and with time and location due to a complex cascade of cellular reactions.}
    \label{fig:thresholds}
\end{figure}

==> figures/vasculature.tex <==
\begin{figure}[b]
    \newcommand\myscale{\scaleppt}
    \setlength\tabcolsep{0pt}
    \centering
    \includegraphics[scale=\scale,scale=\myscale]{\rootpath figures/files/vasculature.pdf}
    \caption[The cerebral vasculature.]{The cerebral vasculature. LEFT: A schematic representation of the cerebrovascular anatomy. Arterial and venous trees connect at the level of the capillaries, respectively carrying oxygen- and glucose-rich (RED) and -deprived (BLUE) blood. Transparent lateral connections refer to the collateral circulation, less or more pronounced across different subjects. RIGHT: A peace of tissue contains many capillaries and cells. Blood perfusion takes place when the \gls{cpp} overcomes the \gls{cvr}. A combination of the \gls{cbf}, \gls{cbv} and \gls{oef} summarizes the access to oxygen and glucose.}
    \label{fig:vasculature}
\end{figure}
